The Hidden Pitfalls of the Cosine Similarity Loss

We show that the gradient of the cosine similarity between two points goes to zero in two under-explored settings: (1) if a point has large magnitude or (2) if the points are on opposite ends of the latent space. Counterintuitively, we prove that optimizing the cosine similarity between points forces them to grow in magnitude. Thus, (1) is unavoidable in practice. We then observe that these derivations are extremely general -- they hold across deep learning architectures and for many of the standard self-supervised learning (SSL) loss functions. This leads us to propose cut-initialization: a simple change to network initialization that helps all studied SSL methods converge faster.

==> Figures/aug_sweep_example.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{Images/augmentations/rotation_example.png}
    \\
    \includegraphics[width=0.4\textwidth]{Images/augmentations/perspectives_example.png}
    \\
    \includegraphics[width=0.4\textwidth]{Images/augmentations/brightness_example.png}
    \caption{Example endpoints for rotation, perspective and brightness sweeps in Fig.~\ref{fig:transform_sweep} on Cifar10. The left (right) column shows the augmentation on the left (right) end of each $x$-axis.}
    \label{fig:sweep_example}
\end{figure}

==> Figures/embedding_dists.tex <==
\begin{figure*}[b!]
    \centering
    \hspace*{-0.2cm}
    \includegraphics[width=1.011\textwidth]{Images/embedding_dists/simclr_embedding_dists.png}
    \\
    \hspace*{-0.22cm}
    \includegraphics[width=1.011\textwidth]{Images/embedding_dists/simsiam_embedding_dists.png}
    \\
    \hspace*{-0.22cm}
    \includegraphics[width=1.011\textwidth]{Images/embedding_dists/byol_embedding_dists.png}
    \caption{Embedding statistics of SimCLR, SimSiam and BYOL during 64 epochs of training.
    \\
    \underline{\textbf{Columns}:} The \underline{$1^\text{st}$ column} shows the mean distance from normalized embedding $z_i$ to its normalized positive embedding $z_j$. The \underline{$2^\text{nd}$ column} shows the mean distance from a normalized embedding $z_i$ to its \emph{closest} normalized negative embedding $z_k$. The \underline{$3^\text{rd}$ column} shows the average embedding norm over the course of training. The \underline{$4^\text{th}$ column} shows the cosine similarity for $z_i$ at epochs $t$ \& $2t$.
    \\
    \underline{\textbf{Rows}:} The \underline{top row} shows SimCLR when optimizing losses $\mathcal{L}^\mathcal{A}$, $\mathcal{L}^{InfoNCE}$, and $\mathcal{L}^\mathcal{R}$. The \underline{middle row} shows SimSiam without the stop-gradient operator and weight-decay 5e-4, with the stop-gradient operator and weight-decay 5e-4 (default), and with the stop-gradient operator and weight-decay $0$. The \underline{bottom row} shows BYOL without the predictor head and weight-decay 5e-4, with the predictor head and weight-decay 5e-4 (default), and with the predictor head and weight-decay 0.}
    \label{fig:embed_dists}
\end{figure*}

==> Figures/transform_sweep.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{Images/augmentations/transform_sweep.pdf}
    \caption{Magnitude of $z_i - z_j$ along $z_i$ (top) and orthogonal to $z_i$ (bottom) as we augment input point $x_i$. The red lines correspond to embeddings from the same control model that was trained with all 6 augmentations while the blue lines represent models that were trained with only the other 5 augmentations (holding out the augmentation in question).}
    \label{fig:transform_sweep}
\end{figure*}

==> Sections/eccv_1_intro.tex <==
\section{Introduction}

Many of the successes of modern deep learning rest on self-supervised learning (SSL) paradigms. These training methods can learn robust, multi-use representations in the absence of labeled data by ensuring that similar (positive) inputs are mapped to nearby locations in embedding space. This is achieved by maximizing the cosine similarity loss between positive embeddings and has proven effective in settings such as unsupervised image recognition~\cite{simclr, simsiam, moco, byol}, segmentation~\cite{dino}, and few-shot learning~\cite{few_shot_text, few_shot_image, few_shot_image_two}. As a result, SSL methods have been extremely well studied, with several theories emerging to describe how optimizing the cosine similarity leads to quality learned representations~\cite{understanding_contr_learn, understanding_contr_learn_2, latent_inversion}. However, to the surprise of the authors of this paper, the properties of the cosine similarity loss -- the commonality across SSL methods -- have seemingly gone unstudied. That is, it is unclear whether the cosine similarity loss has unintended consequences for the optimization process.

Through a simple theoretical analysis, we identify that this is indeed the case: there are two undesirable settings in which the gradient of the cosine similarity goes to 0. That is, even when the representation has not converged, the effective learning rate of a data sample is near zero if (1) its embedding has a large magnitude in the latent space or (2) it is on the opposite side of the latent space from its positive sample. We refer to (1) and (2) as the \emph{Embedding-Norm} effect and the \emph{Opposite-Halves} effect respectively and depict each in Figure~\ref{fig:overview}. We ultimately prove that both effects impose at least a quadratic slowdown on the SSL convergence. These theoretical results are particularly surprising since, under the accepted SSL theory, neither effect is expected to impact the training process \cite{understanding_contr_learn, simsiam_avoid_collapse, latent_inversion, common_stability}.

\begin{figure}[t!]
    \centering
    \includegraphics[trim={0.3cm 5cm 2cm 0},clip,width=\linewidth]{Images/paper_overview.pdf}
    \caption{(\emph{Left}) The SSL embedding pipeline: given two views of the same input, we attract their representations by maximizing the cosine similarity. (\emph{Middle}) Depiction of the embedding-norm effect on latent embedding $z_i$: the effective learning rate decreases as $||z_i||$ grows. (\emph{Right}) Depiction of the opposite-halves effect on $z_i$: the effective learning rate decreases as the angle between $z_i$ and $z_j$ goes to $\pi$.}
    \label{fig:overview} \vspace*{-0.5cm}
\end{figure}

We proceed by verifying the extent to which each occurs in practice. For the opposite-halves effect, we show that although batch-normalization causes positive pairs of embeddings to straddle the origin, this only occurs at the beginning of training and is exceedingly unlikely to impact the training process. Indeed, we see that after a few epochs the opposite-halves effect ceases to appear in SSL latent spaces. Switching to the embedding-norm effect, we prove the surprising fact that maximizing the cosine similarity between two points \emph{must} cause those points to grow in magnitude. This leads to an unfortunate catch-22: SSL methods can only be trained under small embedding norms but optimizing the loss-function grows those same embedding norms. Furthermore, this growth also occurs when minimizing any objective that is itself a function of the cosine similarity (such as the InfoNCE loss between normalized embeddings~\cite{contr_pred_coding}). Importantly, the corresponding derivation is \emph{completely independent} of the SSL architecture, implying that the theory holds across cosine-similarity-based SSL methods. We therefore round out our analysis by verifying that the embedding-norm effect negatively impacts the convergence of \emph{all} tested SSL architectures.

We conclude by proposing \emph{cut-initialization}, a simple change to neural network initialization wherein all weight values are divided by $c>1$. Under our proposed changes, SSL embeddings start at the optimal magnitude and remain at this magnitude for the entire training process, therefore nullifying the embedding-norm effect. We confirm that this improvement holds across SSL optimization schemes, backbone architectures, parameter choices, and datasets, implying that cut-initialization should be implemented in \emph{all} settings where the cosine similarity or InfoNCE losses are minimized. In summary:
\begin{itemize}
    \item We analyze the gradients of the cosine similarity and show several settings where they behave counter-intuitively.
    \item We provide an updated understanding of the distribution of latent features in SSL models, extending previous theoretical analyses to attraction-only models such as SimSiam and BYOL.
    \item We propose \emph{cut-initialization} -- a simple change to network initialization under which all tested SSL methods converge significantly faster.
\end{itemize}
Our code will be made available. \vspace*{-0.2cm}

==> Sections/eccv_2_related_work.tex <==
\section{Preliminaries and Related Work}

\subsection{Self-Supervised Learning Methods}

SSL representations are learned from a dataset without utilizing any labels. This is typically done by obtaining two views (augmented variants) $x_i$ and $x_j$ from an input image $x$ and ensuring that the corresponding embeddings $z_i$ and $z_j$ have high cosine similarity. We will refer to $(x_i, x_j)$ (resp. $(z_i, z_j)$) as `positive' pairs of points (resp. embeddings). The encoder is traditionally a Resnet~\cite{resnet} or ViT~\cite{ViT, dino} followed by several feed-forward layers that are termed the `projector'. Each SSL method then introduces an additional mechanism that prevents the entire learned representation from collapsing to a single point.
Below, we give a summary of the different SSL methods that we use in this paper to verify our theoretical results. Our hyperparameters and other experimental details are specified in Section~\ref{sec:experiment_setup} in the Appendix. \vspace*{0.08cm}

\noindent \textbf{SimCLR.} SimCLR~\cite{simclr} follows from a line of research of contrastive methods for unsupervised image processing \cite{contr_pred_coding, data_efficient_cpc, moco, mocov2, pirl}. Like all of these methods, SimCLR uses repulsive forces to prevent collapse. These \textit{negative} points are all of the other samples in the batch, implying that no two points in a batch can be mapped to the same latent position. We refer to the negative embeddings as $z_k$ and use the notation $k \not\sim i$ to represent the set of negative elements in a batch for embedding $z_i$. We use $\hat{z}$ to represent the unit vector of $z$ and write $\mathbf{z}$ when emphasizing the direction component in an equation. Lastly, $\text{sim}(a, b) = \exp \left( \hat{a}^\top \hat{b} \right) = \exp \left( \frac{a^\top b}{||a|| \cdot ||b||} \right)$ is the exponent of the cosine similarity.

Given this, SimCLR maximizes the cosine similarity between positive embedding pairs and minimizes the LogSumExp of cosine similarities among all negative embedding pairs~\cite{contr_pred_coding}. Thus, the loss for embedding $z_i$ is
\begin{align}
    \label{eq:infonce}
    \mathcal{L}_i(\mathbf{Z}) &= -\log \frac{\text{sim}(z_i, z_j)}{\sum_{k \not\sim i} \text{sim}(z_i, z_k)} \nonumber \\
    &= -\hat{z}_i^\top \hat{z}_j + \log \left[ \sum_{k \not\sim i} \text{sim}(z_i, z_k) \right] = -\underbrace{\hat{z}_i^\top \hat{z}_j}_{\mathcal{L}^\mathcal{A}_i(\mathbf{Z})} + \underbrace{\log \left( S_i \right)}_{\mathcal{L}^\mathcal{R}_i(\mathbf{Z})},
    \vspace*{-0.3cm}
\end{align}
where $S_i = \sum_{k \not\sim i} \text{sim}(z_i, z_k)$ is the sum over the repulsive terms. For clarity, we split the loss term into attraction $\mathcal{L}^\mathcal{A}_i(\mathbf{Z})$ and repulsion $\mathcal{L}^\mathcal{R}_i(\mathbf{Z})$ loss functions\footnote{The result of optimizing the attraction term is that the positive pair of points is pulled closer together. Similarly, optimizing the repulsion term causes the negative point pairs to be pushed apart from each other.}, where index $i$ implies that there is one index $j \neq i$ that is the positive embedding in $\mathbf{Z}$ and all indices $k\neq i, j$ are the negative embeddings. We will refer to $\mathcal{L}^\mathcal{A}_i$ as the \emph{only-attractions} loss and $\mathcal{L}^\mathcal{R}_i$ as the \emph{only-repulsions} loss.
%since the gradients of each component encourage attractions and repulsions respectively among corresponding embeddings. 
Note that $\mathcal{L}^\mathcal{A}_i(\mathbf{Z})$ is simply the negative cosine similarity between $z_i$ and $z_j$.

In SimCLR and other SSL methods, the quality of a learned representation is measured by training classifiers on the learned representations -- if the classifier achieves high accuracy then embeddings corresponding to the same class must be near one another. As is common practice, we use the $k$-nn classifier accuracy which effectively lower-bounds the linear finetuning accuracy~\cite{dinov2}. \vspace*{0.08cm}

 %We also note that virtually every modern SSL method uses the inner product among \emph{normalized} embeddings when calculating the loss values, including but not limited to \cite{moco, simclr, simsiam, byol, protonce, nnclr}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Images/model_diagrams.pdf}
    \caption{Diagrams describing the models used in this paper.}
    \label{fig:diagrams} \vspace*{-0.5cm}
\end{figure}

\noindent \textbf{BYOL and SimSiam.} Surprisingly, BYOL~\cite{byol} and SimSiam~\cite{simsiam} showed that one can focus solely on attractions between similar points without the representation collapsing. Thus, these non-contrastive methods simply optimize the cosine similarity $\mathcal{L}^\mathcal{A}_i$, making them ideal candidates for studying the effects of the cosine similarity objective (we refer to these as \emph{attraction-only} methods).

For these methods, the embedding $z_j$ is obtained via an encoder while $z_i$ goes through an encoder with a connected predictor\footnote{The predictor is a multi-layer feedforward network.}. The gradients during training are then only passed through the embedding $z_i$. In BYOL, the encoder that produces $z_j$ is a moving average \cite{moco} of the $z_i$ encoder with the momentum term set to $\tau=0.99$. Thus, after each training step, we update the weights by $\theta_j' = \tau \theta_j + (1 - \tau) \theta_i$, where $\theta_i$ represents weight in the encoder that produced $z_i$ and $\theta_j$ represents the corresponding weight in the momentum-encoder. In the case of SimSiam, $\tau$ is set to 0, implying that the second encoder is simply a direct copy of the first one. \vspace*{0.08cm}

\noindent \textbf{MoCo and other contrastive methods.} We conclude by discussing the popular SSL methods MoCo~\cite{moco, mocov2, mocov3} and Dino~\cite{dino, dinov2}. All versions of MoCo use a momentum-encoder to obtain the positive embedding $z_j$ and a queue of negative embeddings $z_k$. Whereas MoCo and MoCov2 use a Resnet backbone, MoCov3 uses a transformer-based ViT \cite{ViT} model. Nonetheless, since all versions optimize the InfoNCE loss, our theoretical discussions apply across MoCo versions. Similarly, we note that our results also hold for other contrastive methods like SwAV~\cite{swav}, ProtoNCE~\cite{protonce}, nnCLR~\cite{nnclr}, and Propos~\cite{learning_representation_clustering} which use clustering or prototypes for their positive/negative samples but still have an inner product among normalized embeddings in their loss calculations. Dino, on the other hand, optimizes the cross-entropy between unnormalized embeddings without using inner products. As such, our theoretical discussions do not apply to Dino.

\subsection{Theory of Self-Supervised Learning}
\label{ssec:theory_rel_work}

Due to the success of SSL models, there has been significant research investigating how they learn so effectively without labeled data. As was discussed in~\cite{contr_pred_coding}, one can interpret the InfoNCE loss function as trying to learn a classifier that can distinguish every sample from every other sample in the dataset. However, this does not tell the whole story -- why do samples from the same class end up near one another? To this end, the seminal work of~\cite{understanding_contr_learn} showed that contrastive learning must satisfy two requirements: all positive pairs must be near one another (alignment) and all negative samples must spread evenly over the hypersphere (uniformity). They then argued that satisfying these requirements leads to classes grouping together. After \cite{understanding_contr_learn}, there has been an implicit agreement that the latent representation on the hypersphere is all that one must consider when analyzing SSL models~\cite{provable_contr_guarantees, common_stability}. We discuss the incompleteness of this viewpoint in Section~\ref{ssec:consequences}. We furthermore note that there has not been an extension of the analysis in~\cite{understanding_contr_learn} to attraction-only models like BYOL and SimSiam, which we provide in Section~\ref{sec:verification}.

Expanding on this theoretical blueprint, subsequent works have sought to formalize the learning capacity of contrastive methods. For example, \cite{geom_contrastive_loss} showed that a geodesic contrastive loss leverages the hyperspherical interpretation of \cite{understanding_contr_learn} and leads to better class separation. Additionally, \cite{latent_inversion} showed that contrastive models can recover latent features by inverting the implicit generative model. Still other works \cite{provable_contr_guarantees, understanding_contr_learn_2} discuss the effect of the data-augmentation and the training procedure on the generalizability of contrastive models. Since all of the above works focused on contrastive tasks, it remains an open question what theoretical guarantees can be made of attraction-only models.

Indeed, much of the research studying SimSiam and BYOL has focused on specific components of their architectures. For example, \cite{simsiam_avoid_collapse} showed that the predictor is essential for attraction-only models to prevent collapse. Furthermore, \cite{dim_collapse_ssl, BYOL_orthogonality, direct_pred} show that the predictor is serving as a low-rank approximator and suggest replacing it with dimensionality reduction methods. The relationship between SSL and dimensionality reduction is further studied in \cite{ssl_dim_reduction}. Finally, \cite{duality_contr_non-contr} discussed how to improve SimCLR by incorporating non-contrastive methods.

\subsection{Normalization, Initialization, and Regularization}

Weight decay is implemented by adding a loss term that penalizes large weights, i.e. $\mathcal{L}'(\mathbf{Z}; \theta) = \mathcal{L}(\mathbf{Z}; \theta) + \lambda \sum_l ||\theta_l||^2$, where $\theta_l$ corresponds to the weights in layer $l$ of the encoder and $\lambda$ is the weight-decay hyperparameter\footnote{We note that BYOL and SimSiam both use higher weight-decay ($\lambda = 5$e-$4$) than SimCLR ($\lambda = 1$e-$6$).}. Batch normalization is a network layer that rescales the features to have 0-mean and unit variance and includes learned parameters that can further augment the mean and variance as needed. We note that applying batch-norm on the encoder's output will therefore redistribute the learned features around the hypersphere. It is an open question why SSL models require \ltwo-normalization\footnote{We use the terms weight-decay and \ltwo-normalization interchangeably as they are equivalent under SGD~\cite{decoupled_l2}. We will often say norm as shorthand for normalization.} \cite{direct_pred, byol, common_stability_comment} in order to converge. Our work resolves this question both in theory and in practice.

There has been significant study into the effects of normalizations and initializations on the convergence of neural networks ~\cite{3_mechanisms_weight_decay, decoupled_l2, weight_norm}. A related work to ours is \cite{l2_norm_effective_lr}, where it was shown that \ltwo-normalization affects the effective learning rate of a network. Although similar in principle, we note that the results in \cite{l2_norm_effective_lr} are \emph{completely independent} of our analysis in Section~\ref{sec:embeddings}.

Lastly, regarding the gradients of the cosine similarity, the most related work to ours is~\cite{normface}. The authors show that replacing the softmax's inner products with the cosine similarity resolves distributional issues in the softmax function. Our work differs from theirs as we instead resolve the cosine similarity's pitfalls. \vspace*{-0.25cm}




%\input{Figures/embedding_dists}

%When discussing `embeddings', we are referring to the latent space being learned by the projection and prediction heads. Specifically, we are referring to SimCLR's projector and SimSiam and BYOL's predictors. When performing classification experiments using the frozen features, we are instead using the output of the Resnet-18 as input to a classifier. We refer to these as `linear classifier' experiments. To be consistent with the literature, we also sometimes report $k$nn-classifier accuracies to verify the quality of a learned representation.

% \subsection{Notes}
% \begin{itemize}
%     \item Things to note for later:
%     \begin{itemize}
%         \item PIRL has a plot showing that their embeddings ARE invariant to the transformation somehow??
%     \end{itemize}
%     \item Papers that say that we use repulsions to avoid collapsing:
%     \begin{itemize}
%         \item BYOL paper, section 3 \cite{byol}
%         \item Understanding Dimensional Collapse in Contrastive Self-Supervised Learning

%     \end{itemize}
%     \item Papers that say that we use attractions to learn an invariant representation:
%     \begin{itemize}
%         \item \cite{disentangled_imaging}
%     \end{itemize}
% \end{itemize}


==> Sections/eccv_3_method_embedding_analysis.tex <==

\section{Theoretical Analysis}

\subsection{Gradients of the Cosine Similarity}
\label{sec:embeddings}

We now present the gradients of the Euclidean cosine similarity:

\begin{proposition}
    \label{prop:cos_sim_grads}
    Let $z_i$ and $z_j$ be two embeddings and define $\mathcal{L}_i^\mathcal{A}(\mathbf{Z}) = -\hat{z}_i^\top \hat{z}_j$. Let $\phi_{ij}$ be the angle between $z_i$ and $z_j$. Then the gradient of $\mathcal{L}_i^\mathcal{A}(\mathbf{Z})$ w.r.t. $z_i$ is
    \[ \nabla_i^\mathcal{A} = \frac{1}{||z_i||} \left(\mathbf{I} - \frac{z_i z_i^\top}{||z_i||^2} \right) \frac{\mathbf{z}_j}{||z_j||} = \left( \frac{\hat{z}_j}{||z_i||} \right)_{\perp z_i} \]
    where $a_{\perp b}$ is the component of $a$ orthogonal to $b$.
    This has norm $||\nabla_i^\mathcal{A}|| = \frac{\sin(\phi_{ij})}{||z_i||}$.
\end{proposition}
We prove this in~\ref{prf:prop_grad_grows} in the Appendix.
\vspace*{0.05cm}

This has an easy interpretation. Consider that the linear operator $\mathbf{I} - \frac{z_i z_i^\top}{||z_i||^2}$ acts as a projection onto the subspace orthogonal to $\vec{z}_i$. Thus, our attraction gradient takes the unit vector $\hat{z}_j$, projects it onto the plane orthogonal to $\vec{z}_i$, and then scales this inversely by $||z_i||$. We visualize the projection in Figure~\ref{fig:embedding_visualizations} where the purple plane represents the codomain of the projection operator. We refer to this as the \emph{tangent space} at $z_i$. Furthermore, note that the gradient's magnitude acts as a direct scalar on the learning rate since $\gamma \vec{\nabla}_i = (\gamma ||\nabla_i||) \hat{\nabla}_i$.

\begin{figure}
    \centering
    \includegraphics[trim={5cm 4.2cm 12cm 2.7cm},clip,width=0.27\linewidth]{Images/contr_attractions.pdf}
    % \captionof{figure}{The gradients w.r.t. $z_i$ in Proposition~\ref{prop:cos_sim_grads} and Corollary~\ref{cor:grad_grows} exclusively exist in the tangent space at $\vec{z}_i$.}
    % \label{fig:grad_visualization}
    \quad \quad \quad
    \includegraphics[trim={1cm 4.5cm 8.5cm 4.5cm},clip,width=0.6\linewidth]{Images/growing_embeddings.pdf}
    % \captionof{figure}{A visualization of the growing embeddings in Corollary~\ref{cor:embeddings_grow}. Blue points represent $z_i$ at iterations $t = 1, 2, 3$. Yellow points represent $z_i'$, i.e. the result of each step of gradient descent.}
    % \label{fig:growing_embeddings}
    \caption{\emph{Left}: The gradients w.r.t. $z_i$ in Proposition~\ref{prop:cos_sim_grads} and Corollary~\ref{cor:grad_grows} exclusively exist in the tangent space at $\vec{z}_i$. \emph{Right}: A visualization of the growing embeddings in Corollary~\ref{cor:embeddings_grow}. Blue points represent $z_i$ at iterations $t = 1, 2, 3$. Yellow points represent $z_i'$, i.e. the result of each step of gradient descent.}
    \label{fig:embedding_visualizations} \vspace*{-0.5cm}
\end{figure}

As a consequence of Prop.~\ref{prop:cos_sim_grads}, we also see that maximizing the cosine similarity can \emph{only grow the embeddings}:
\begin{corollary}
    \label{cor:embeddings_grow}
    Let $z_i$ and $z_j$ be positive embeddings with angle $\phi_{ij}$. Let $z_i' = z_i + \frac{\gamma}{||z_i||}(z_j)_{\perp z_i}$ be the embedding after applying the Prop.~\ref{prop:cos_sim_grads} gradients to $z_i$ via a single step of gradient descent with learning rate $\gamma$. Then
    \[ ||z_i'|| \geq ||z_i||, \]
    with equality if and only if $\sin \phi_{ij} = 0$.
\end{corollary}
\begin{proof}
    Since $z_i$ and $(z_j)_{\perp z_i}$ are orthogonal, $||z_i'||_2^2 = ||z_i||^2 + \frac{\gamma^2}{||z_i||^2}||(z_j)_{\perp z_i}||^2$. The second term is positive if $\sin \phi_{ij} > 0$. Figure~\ref{fig:embedding_visualizations} visualizes this.
\end{proof}

The results in Prop.~\ref{prop:cos_sim_grads} and Corollary~\ref{cor:embeddings_grow} reveal the cosine similarity's inevitable catch-22: we require small embeddings to optimize the cosine similarity but optimizing the cosine similarity increases the embeddings.

We note that these results depend neither on the existence of $\mathbf{X}$ nor on the embedding pipeline -- they simply assume that there exists some distribution $\mathbf{Z}$ that we apply the cosine similarity onto. As a result, the dynamics in Prop.~\ref{prop:cos_sim_grads} and Corollary~\ref{cor:embeddings_grow} apply, in theory, to every setting where the cosine similarity is being optimized. Furthermore, these results also hold for the mean squared error between normalized embeddings. Namely, let $\mathcal{L}_{MSE} = ||\hat{z}_i - \hat{z}_j||_2^2$. Then it is known that $\mathcal{L}_{MSE} = 2 - 2\hat{z}_i^\top \hat{z}_j$, implying that the normalized mean squared error's gradients are equivalent to those of the negative cosine similarity's~\cite{byol}.

\subsection{InfoNCE Gradients}

The InfoNCE gradient has a similar structure to the cosine similarities:

\begin{corollary}
    \label{cor:grad_grows}
    Let $\mathbf{Z}$ be a set of $b$ embeddings in $\mathbb{R}^d$, with $z_i$ corresponding to the $i$-th row of $\mathbf{Z}$. Let $\mathcal{L}_i(\mathbf{Z}) = \mathcal{L}_i^\mathcal{A}(\mathbf{Z}) + \mathcal{L}_i^\mathcal{R}(\mathbf{Z})$. Then the gradient of $\mathcal{L}_i(\mathbf{Z})$ w.r.t. $z_i$ is
    \begin{equation}
        \label{eq:infonce_grads}
        \nabla^{InfoNCE}_i = \frac{1}{||z_i||} \left[ \left( \hat{z}_j \right)_{\perp z_i} + \sum_{k \not\sim i} \left( \hat{z}_k \cdot \frac{\text{\emph{sim}}(z_i, z_k)}{S_i} \right)_{\perp z_i} \right].
    \end{equation}\vspace*{-0.2cm}
    \label{cor:infonce_grads}
\end{corollary}
We prove this in Section~\ref{prf:cor_grad_grows} in the Appendix. In essence, because the InfoNCE loss is a function of the cosine similarity, the chain rule implies that its gradients have similar properties to the cosine similarity's. Specifically, just like those of $\mathcal{L}_i^\mathcal{A}$, the gradients of $\mathcal{L}_i^\mathcal{R}$ have the properties that (1) they are inversely scaled by $||z_i||$, (2) they are only defined in $z_i$'s tangent space, and (3) optimizing the repulsions cause the embeddings to grow\footnote{The primary difference is that the repulsive gradients have a weighted average over all the negative samples $z_k$. We note that this weighted average over a set of unit vectors leads to the repulsive force being smaller than the attractive one.}. Since the InfoNCE loss is the sum of $\mathcal{L}_i^\mathcal{A}$ and $\mathcal{L}_i^\mathcal{R}$, these properties all extend to the InfoNCE loss as well. 

\subsection{The Zero Gradient Settings}
\label{ssec:consequences}

At this point in our discussion, the cosine similarity's gradient is merely a curiosity. However, the important details lie in its magnitude: $||\nabla^{\mathcal{A}}_i || = \frac{\sin \phi_{ij}}{||z_i||}$. Specifically, the gradient of the cosine similarity (and, by Corollary~\ref{cor:infonce_grads}, the InfoNCE loss) goes to zero when an embedding has large norm or is across the latent space from its positive-pair counterpart. This ultimately leads to a super-linear slowdown on the convergence rate:

\begin{theorem}
    Let $z_i$ and $z_j$ be positive embeddings with equal norm, i.e. $||z_i|| = ||z_j|| = \rho$. Let $z_i' = z_i + \frac{\gamma}{\rho}(z_j)_{\perp z_i}$ and $z_j' = z_j + \frac{\gamma}{\rho}(z_i)_{\perp z_j}$ be the embeddings after maximizing the cosine similarity via a single step of gradient descent with learning rate $\gamma$. Then the change in cosine similarity is bounded from above by:
        \begin{equation}
            \label{eq:thm_statement}
            \hat{z}_i'^\top \hat{z}_j' - \hat{z}_i^\top \hat{z}_j < \frac{2 \gamma \sin^2 \phi_{ij}}{\rho^2}.
        \end{equation}
    
    \label{thm:convergence_rate}
\end{theorem}
The proof can be found in Section \ref{prf:thm_convergence_rate} of the Appendix. \vspace*{0.2cm}

\noindent \begin{minipage}{0.35\textwidth}
To visualize this slowdown, we create sets of random samples of 500 pairs of points in $\mathbb{R}^{20}$ such that each set of samples has different mean embedding norms and $\phi_{ij}$ values. We then apply the gradients in Prop.~\ref{prop:cos_sim_grads} onto each set of points until the average cosine similarity exceeds $0.999$ to study how these terms will affect convergence. The resulting convergence times are shown in Figure~\ref{fig:convergence_rate}.
\end{minipage}
\quad
\begin{minipage}{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Images/bounds.pdf}
    \captionof{figure}{Visualizing the results in Theorem~\ref{thm:convergence_rate}: The effect of the embedding norm and angle between positive samples on the convergence rate.}
    \label{fig:convergence_rate}
\end{minipage} \vspace*{0.2cm}

We find that (1) both terms indeed impose a super-linear slowdown on the convergence time, and (2) having large embedding norms is \emph{significantly} worse for optimization ($\sim\!\!100\times$ slowdown) than having large angles between positive pairs ($\sim\!2\times$ slowdown). We now present each effect formally and discuss its relationship with established SSL theory (Section~\ref{ssec:theory_rel_work}): \vspace*{0.08cm}

\noindent \textbf{The Embedding-Norm Effect.} Consider two latent distributions $\mathbf{Z}$ and $\mathbf{Z}'$ where $\mathbf{Z}' = c \mathbf{Z}$. These embeddings are identical when projected onto the hypersphere and therefore correspond to equivalently `good' representations~\cite{understanding_contr_learn}. Nonetheless, by Prop.~\ref{prop:cos_sim_grads} and Theorem~\ref{thm:convergence_rate}, if $c \gg 1$ then our ability to optimize $\mathbf{Z}'$ falls dramatically. Thus, while the hyperspherical projection defines the quality of the learned representation, \emph{the distribution in ambient space controls how quickly this representation can be updated.} We refer to this as the \emph{Embedding-Norm} effect. To our knowledge, this is the first result showing that one cannot only consider the SSL representation over the hypersphere. \vspace*{0.08cm}

\noindent \textbf{The Opposite-Halves Effect.} Although it may be obvious in hindsight\footnote{$\frac{d\, (-\cos x)}{dx} = \sin x$.} that the gradient depends on $\sin \phi_{ij}$, intuition says that higher loss values should incur correspondingly larger gradients. Despite this, \emph{positive embeddings on opposite poles of the hypersphere incur the largest loss but are barely attracted to each other}. Indeed, if two positive samples have angle $0 < \varepsilon < \pi$ while two other positive samples have angle $\pi - \varepsilon$, they will both experience the same amount of attraction. Figure~\ref{fig:convergence_rate} shows that the resulting slowdown in training becomes significantly worse as $\varepsilon \rightarrow 0$. We refer to this as the \emph{Opposite-Halves} effect.

==> Sections/eccv_4_verification.tex <==
\section{The Practical Consequences of the Cosine Similarity}
\label{sec:verification}

The theoretical discussion in Section~\ref{sec:embeddings} only relied on the existence of $\mathbf{Z}$ and was therefore independent of the inputs $\mathbf{X}$ or the embedding pipeline. We now verify whether each effect practically impacts SSL training dynamics or, indeed, whether the effect occurs at all.

\subsection{Embedding-Norm Effect in Practice}
\label{ssec:emb_norm_verification}

\input{Figures/embedding_mags}
\begin{table}
    \centering
    \fontsize{6.5pt}{6.5pt}\selectfont
    %\hspace*{-0.45cm}
    \begin{tabular}{lccc}
        \multicolumn{4}{c}{\small{Embedding Magnitudes}} \\
        \midrule
        \makecell{Weight\\Decay} & SimCLR & SimSiam & BYOL \\
        \midrule
        $\lambda=$ 5e-2 & 0.0 & 0.0 & 0.0 \\
        $\lambda=$ 5e-3 & 0.10 & 0.47 & 0.45 \\
        $\lambda=$ 5e-4 & 0.41 & 0.81 & 0.70 \\
        $\lambda=$ 5e-6 & 13.5 & 24.5 & 23.2 \\
        $\lambda=$ 0 & 16.4 & 31.4 & 30.1 
    \end{tabular}
    \;
    \begin{tabular}{lccc}
        \multicolumn{4}{c}{\small{$k$nn Accuracies}} \\
        \midrule
        \makecell{Weight\\Decay} & SimCLR & SimSiam & BYOL \\
        \midrule
        $\lambda=$ 5e-$2$ & 10.0 & 10.0 & 10.0 \\
        $\lambda=$ 5e-3 & 54.0 & \underline{57.2} & \textbf{78.0} \\
        $\lambda=$ 5e-4 & \textbf{81.3} & \textbf{73.3} & \underline{74.3} \\
        $\lambda=$ 5e-6 & \underline{75.7} & 48.2 & 47.8 \\
        $\lambda=$ 0 & 75.3 & 47.9 & 47.3
    \end{tabular}
    \;
    \begin{tabular}{lccc}
        \multicolumn{4}{c}{\small{$k$nn Accuracies}} \\
        \midrule
        \makecell{Learning\\Rate} & SimCLR & SimSiam & BYOL \\
        \midrule
        $\gamma =$ 1.8 & 58.8 & 10.0 & 10.0 \\
        $\gamma =$ 0.6 & \textbf{81.3} & \underline{60.2} & \textbf{82.6} \\
        $\gamma =$ 0.2 & \underline{71.2} & \textbf{73.6} & \underline{72.5} \\
        $\gamma =$ 0.067 & 45.8 & 37.3 & 38.3 \\
        $\gamma =$ 0.022 & 36.7 & 35.5 & 35.8 
    \end{tabular}

    \caption{(a) \& (b): Effect of weight-decay parameter $\lambda$ on SSL embedding magnitudes \& $k$nn-accuracies, respectively. (c): Effect of learning-rate parameter $\gamma$ on $k$nn-accuracies. Evaluation is done on Cifar10 after 128 epochs of training.}
    \label{tbl:weight_decay}
\end{table}

To see whether the embedding-norm effect occurs, we plot the average embedding magnitudes for SimCLR, SimSiam, and BYOL on Cifar10\footnote{The choice of Cifar10 is arbitrary as the effects are independent of the dataset.}~\cite{cifar10} in Figure~\ref{fig:embed_mags}. The left-most plot shows that the SimCLR embedding magnitudes monotonically increase if we are optimizing either the attractions or the repulsions. We also confirm that optimizing the attractions causes the embedding norms to grow \emph{faster} than optimizing the repulsions. Thus, the embedding norms do grow as a result of optimizing either the cosine similarity or the InfoNCE loss.

We next turn to the question of whether higher embedding norms lead to slower convergence in practice. To this end, Table~\ref{tbl:weight_decay} shows the relationships between the weight-decay, the embedding norm, and the learning rate with respect to the classification accuracy on Cifar10. We find that, after about 100 epochs of training, the weight decay parameter can control for the mean embedding magnitudes\footnote{Higher weight decay $\rightarrow$ small embedding norms after a sufficient number of epochs.}. We then see that these magnitudes directly correlate with the $k$-nn accuracies, where smaller embeddings lead to improved classification accuracy. Additionally, the embedding magnitudes and the learning rate affect the accuracies in a similar fashion: each parameter has a `goldilocks-zone' under which the model converges well but, outside this range, the network either converges slowly or the training is unstable.

Thus, we conclude that (1) the embedding-norm effect is unavoidable in practice, and (2) modern SSL methods address it by applying weight-decay. This resolves the open question of why SSL models require higher weight-decay than non-supervised methods~\cite{byol, direct_pred, common_stability_comment}. However, we point out that the \ltwo-norm is a band-aid rather than a full solution to the embedding-norm effect. Specifically, as the network weights grow smaller, the \ltwo-normalization has diminishing returns. It is therefore unclear how many epochs are wasted while weight-decay is shrinking the embedding magnitudes. Indeed, due to the learning rate schedule many SSL models use, the first epochs of training are the most costly to miss.

\subsection{Opposite-Halves Effect in Practice}
\label{ssec:opp_halves_effect}

We now turn to evaluating how much the opposite-halves effect plays a role in SSL training. Referring back to Figure~\ref{fig:convergence_rate}, we see that it is most impactful when the angle between positive embeddings is close to $\pi$, i.e. $\phi_{ij} > \pi - \varepsilon$ for $\varepsilon \rightarrow 0$. The following result shows that this is exceedingly unlikely in high-dimensions:
\begin{proposition}
    \label{prop:unlikely_opp_halves}
    Let $x_i, x_j \sim \mathcal{N}(0, \mathbf{I})$ be $d$-dimensional, i.i.d. random variables and let $0 < \varepsilon < 1$. Then \vspace*{-0.1cm}
    \begin{equation}
    \label{eq:opp_halves_unlikely}
    \mathbb{P}\left[ \frac{x_i^\top x_j}{||x_i|| \cdot ||x_j||} \geq 1 - \varepsilon \right] \leq \frac{1}{2d(1-\varepsilon)^2}.
    \end{equation}\vspace*{-0.3cm}
\end{proposition}
We prove this in Section~\ref{prf:prop_opp_halves} of the Appendix.

Thus, the theory suggests that the opposite halves effect should not have a strong impact on SSL convergence. To check this, we plot the rate at which two positive pairs have angle greater than $\frac{\pi}{2}$ in Table~\ref{tbl:opposite_half_effect}. There, we see that positive pairs are on opposite ends of the latent space approximately $5\%$ and $25\%$ of the time during the first epoch of SimCLR and BYOL/SimSiam, respectively. To visualize why this happens more for attraction-only embeddings, we train SimCLR and BYOL with a $2$-dimensional projection/prediction latent space (as is done for MoCo in~\cite{understanding_contr_learn}) and draw lines between positive samples in Figure~\ref{fig:2d_latent_spaces}. SimCLR performs as expected -- it distributes the embeddings across the latent space and keeps positive samples close together. However, Figure~\ref{fig:2d_latent_spaces} suggests that BYOL begins by concentrating its embeddings at antipodal points on the hypersphere and does not spread out evenly from there. Drawing from \cite{byol_batchnorm, byol_without_batch_statistics, simsiam}, we attribute this to the batch-normalization that is present in BYOL and SimSiam's projection/prediction heads\footnote{Consider what happens if the distribution has collapsed to a single point right before the batch-normalization layer. Since batch-normalization subtracts the mean and divides by the variance, the single collapsed cluster becomes chaotically distributed across the latent space~\cite{byol_batchnorm}. Thus, batch-normalized models cannot collapse to a single point.}. \vspace*{0.1cm}

\noindent \begin{minipage}{0.45\textwidth}
    \fontsize{7pt}{7pt}\selectfont
    \centering
    \begin{tabular}{lrcc}
    Model & Dataset & \makecell{Effect Rate\\Epoch 1} & \makecell{Effect Rate\\Epoch 16} \\
    \midrule
    \multirow{2}{*}{SimCLR} & Imagenet-100 & 2\% & 0\%  \\
    & Cifar-100 & 11\% & 1\% \\
    \cmidrule{1-4}
    \multirow{2}{*}{SimSiam} & Imagenet-100 & 26\% & 1\% \\
    & Cifar-100 & 21\% & 0\% \\
    \cmidrule{1-4}
    \multirow{2}{*}{BYOL} & Imagenet-100 & 28\% & 1\% \\
    & Cifar-100 & 20\% & 0\% \\
    \end{tabular}
    \captionof{table}{Rate at which the cosine-similarity between positive samples is $<0$; i.e. rate of the opposite-halves effect during training.}
    \label{tbl:opposite_half_effect}
\end{minipage}
\quad \quad
\begin{minipage}{0.5\textwidth}
    \centering
    \includegraphics[width=0.95\linewidth]{Images/positive_pairs.png}
    \captionof{figure}{Lines between positive samples in 2D latent space during training. The color goes from red to blue as the cos. sim. goes from $-1$ to $1$.}
    \label{fig:2d_latent_spaces} \vspace*{0.1cm}
\end{minipage}

Putting these pieces together explains why SimSiam and BYOL have a higher rate of the opposite-halves effect at the start of training. Since they only optimize attractions, they must begin by concentrating embeddings together. Due to batch-normalization, this concentration occurs in several clusters that straddle the origin. Thus, some positive pairs will necessarily have an angle greater than $\frac{\pi}{2}$ at the beginning of training (seen in the `Epoch 1' row of Figure~\ref{fig:2d_latent_spaces}).

We point out, however, that very early into training (epoch 16), every method has a rate of effectively 0 for the opposite-halves effect. This is visualized in Figure~\ref{fig:2d_latent_spaces}, where the learned representations at epoch 128 have very few `red' lines\footnote{Interestingly, Figure~\ref{fig:2d_latent_spaces} also implies that attraction-only methods never reach uniformity over the latent space.}. Furthermore, the rates in Table~\ref{tbl:opposite_half_effect} measure how often $\phi_{ij} > \frac{\pi}{2}$: the absolute weakest version of the opposite-halves effect. If we instead count the number of times that $\phi_{ij} > \frac{7\pi}{8}$ (the range where the opposite halves effect could start mattering according to Figure~\ref{fig:convergence_rate}), then it occurs 0 times across all the experiments in Table~\ref{tbl:opposite_half_effect}. Thus, it is clear that while some weak variant of the opposite-halves effect must occur at the beginning of training, it does not have a strong impact on the convergence dynamics and, in either case, disappears quite quickly. For completeness, Section~\ref{app:new_loss} in the Appendix discusses how to remedy the opposite-halves effect if it is found to slow down convergence.


==> Sections/eccv_5_all_experiments.tex <==
\section{Mitigating the Embedding-Norm Effect}
\label{sec:norm_experiments}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.85\textwidth]{Images/initializations/init_experiments.png}
    \caption{The effect of cut-initialization on Cifar10 SSL representations. $x$-axis and embedding norm's $y$-axis are log-scale. $\lambda=5$e$-4$ in all experiments.}
    \label{fig:cut_experiments} \vspace*{-0.7cm}
\end{figure}

The previous sections showed that the embedding-norm effect occurs in SSL models and that weight decay eventually remedies it. Rather than waiting for the weight-decay to shrink the embedding norms, we propose \emph{cut-initialization}: an initialization scheme where we divide each layer's weights with cut-constant $c>1$ before training. The remainder of the paper verifies cut-initialization's effectiveness across datasets, SSL models, backbone architectures, and loss functions. We emphasize that our theoretical observations are independent of these parameters and, therefore, we are simply showcasing the wide range of settings in which our theoretical analysis (and therefore cut-initialization) applies.

To get a preliminary intuition for cut-initialization's impact on the convergence, we plot the effect of the cut constant on the embedding norms and accuracies over training in Figure~\ref{fig:cut_experiments}\footnote{To make the effect more apparent, we use weight-decay $\lambda=5e-4$ in all models.}. We see that dividing the network's weights by $c>1$ leads to immediate convergence improvements in all models. Furthermore, this effect degrades gracefully: as $c > 1$ becomes $c < 1$, the embeddings stay large for longer and, as a result, the convergence is slower. We also see that cut-initialization has a more pronounced effect in attraction-only models -- a trend that remains consistent throughout the experiments.

We now refer to Tables~\ref{tbl:simclr_wd_cut} and \ref{tbl:simsiam_wd_cut} to study the relationship between the cut-constant and the weight-decay. Specifically, we analyze the classification accuracy after 100 epochs\footnote{We use a Resnet-18 backbone with batch-size 512 for Table~\ref{tbl:simclr_wd_cut} and a Resnet-50 backbone with batch-size 128 for Table~\ref{tbl:simsiam_wd_cut}.} and see that, in both the contrastive and non-contrastive settings, pairing cut-initialization with weight decay accelerates the training process. While this benefit peaks around $c=3$ in the contrastive setting, the non-contrastive paradigm seems incredibly resistant to both high cut-constants and large-weight decays. Based on these results, we default to cut-constant $c=3$ for contrastive methods and $c=9$ for non-contrastive ones.

Table~\ref{tbl:accuracies} then evaluates the effectiveness of cut-initialization on full training runs\footnote{Due to lack of compute, we use a batch-size of 128 with the Resnet50 backbone, indicated by the asterisk. SimCLR state-of-the-art uses batch-sizes $>$1K.}. The immediate takeaway is that cut-initialization essentially guarantees faster convergence and sometimes leads to higher final accuracies. Since Table~\ref{tbl:accuracies}'s purpose is to evaluate cut-initialization, we leave all other model parameters at their defaults. However, we note that modifying the weight decay and learning in tandem with the cut constant would likely lead to further accuracy improvements. Lastly, Table~\ref{tbl:accuracies} verifies that accuracy at 100 epochs is a valid indicator of downstream performance, bolstering the previous experimental sweeps. 

\begin{table}[t!]
    \centering
    \fontsize{7pt}{7pt}\selectfont
        \begin{tabular}{cr cc ccc ccc ccc}
        \toprule
        & & \multicolumn{2}{c}{Cifar10} & \multicolumn{3}{c}{Cifar100} & \multicolumn{3}{c}{Imagenet-100} & \multicolumn{3}{c}{\makecell{Modified\\Flowers}} \\
        \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-13}
        \vspace*{0.05cm}
        & & \multicolumn{2}{c}{Epoch} & \multicolumn{3}{c}{Epoch} & \multicolumn{3}{c}{Epoch} & \multicolumn{3}{c}{Epoch} \\ 
        & & \makecell{100} & \makecell{500} & \makecell{100} & \makecell{300} & \makecell{500} & \makecell{100} & \makecell{300} & \makecell{500} & \makecell{100} & \makecell{300} & \makecell{500} \\
        \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-13}
        \multirow{2}{*}{SimCLR$^*$} & Default & 75.7 & 85.2 & 33.9 & 48.1 & 51.9 & 44.6 & 55.9 & 59.4 & 18.9 & 28.3 & 35.8 \\ % cifar100 33.2
        & Cut ($c=3$) & 79.6 & 86.1 & 42.3 & 50.8 & 52.6 & 46.7 & 58.1 & 60.9 & 23.7 & 50.8 & 65.3 \\ % cifar100 42.3 & 
        \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-13}
        \multirow{2}{*}{SimSiam} & Default & 67.1 & 87.0 & 23.7 & 50.1 & 58.6 & 33.6 & 61.1 & 62.0 & 15.3 & 16.5 & 16.9 \\
        & Cut ($c=9$) & 77.7 & 89.0 & 41.1 & 59.4 & 61.7 & 52.9 & 63.7 & 67.2 & 15.9 & 27.6 & 38.5 \\
        \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-7} \cmidrule(l{2pt}r{2pt}){8-10} \cmidrule(l{2pt}r{2pt}){11-13}
        \multirow{2}{*}{BYOL} & Default & 69.5 & 88.2 & 18.8 & 53.5 & 61.9 & 26.0 & 65.8 & 67.7 & 16.1 & 17.4 & 17.1 \\
        & Cut ($c=9$) & 82.2 & 88.6 & 46.2 & 62.4 & 61.4 & 54.2 & 68.7 & 68.6 & 15.9 & 27.6 & 43.1 \\
        \bottomrule
        \end{tabular}
    \caption{$k$-nn accuracies for default and cut-initialized training.}\vspace*{-.7cm}
    \label{tbl:accuracies}
\end{table}
% simsiam 300 flowers: 16.5 and 27.2
% byol 300 flowers: 17.4 and 27.6

We take a moment to discuss the modified flowers dataset in Table~\ref{tbl:accuracies}. The original Flowers102 dataset \cite{flowers} is nearly impossible for self-supervised image recognition since (a) it only has 10 training images for each of its 102 classes and (b) many of these class differences come down to color distributions, i.e. SSL image augmentations will cross-contaminate the class features. Indeed, none of our tested SSL models are able to learn appropriate representations on the default Flowers102 dataset. We therefore create a new training split using the supplementary imbalanced class examples. Each class in our resulting \emph{modified-flowers} dataset has between 50 and 250 samples, implying a long-tailed data distribution~\cite{long-tail-survey}. This still proves challenging for the default models: SimCLR, SimSiam and BYOL all struggle to learn appropriate class distributions. Despite this, incorporating cut-initialization allows the models to penetrate into a lower loss setting and obtain $k$-nn accuracies that are roughly $25\%$ higher. Thus, not only does cut-initialization accelerate training, it can sometimes facilitate it entirely.

It remains to show that cut-initialization works across SSL models and backbone architectures. To this end, Table~\ref{tbl:accuracies} shows that cut-initialization still provides the expected boost in performance for MoCov2 (which incorporates a negative-sample queue into the SSL pipeline) and for MoCov3 (which uses a ViT-s trasnformer backbone). We furthermore point out that Dino, which does not have a normalized inner product in its loss function, does \emph{not} benefit from cut-initialization. This evidences that cut-initialization's success can be attributed to our theoretical analysis: using cut-initialization in theoretically unmotivated settings no longer has a positive impact on training. \vspace*{0.3cm}

% OLD RESULTS
% \begin{table}
%     \centering
%     \fontsize{8pt}{8pt}\selectfont
%         \begin{tabular}{cr cc cc}
%         \toprule
%         & & \multicolumn{2}{c}{Cifar10} & \multicolumn{2}{c}{Cifar100} \\
%         \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-6}
%         & & \makecell{Acc. \!\!@ \!100\\Epochs} & \makecell{Acc. \!\!@ \!500\\Epochs} & \makecell{Acc. \!\!@ \!100\\Epochs} & \makecell{Acc. \!\!@ \!500\\Epochs} \\
%         \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-6}
%         \multirow{2}{*}{SimCLR} & Default & 75.7 & 85.2 & 37.4 & 49.1 \\
%         & Cut ($c=3$) & 79.6 & 86.1 & 42.3 & 51.6 \\
%         \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-6}
%         \multirow{2}{*}{SimSiam} & Default & 67.1 & 87.0 & 33.4 & 58.2 \\
%         & Cut ($c=9$) & 77.7 & 89.0 & 40.8 & 60.0 \\
%         \cmidrule(l{2pt}r{2pt}){1-2} \cmidrule(l{2pt}r{2pt}){3-4} \cmidrule(l{2pt}r{2pt}){5-6}
%         \multirow{2}{*}{BYOL} & Default & 69.5 & 88.2 & 35.5 & 58.6 \\
%         & Cut ($c=9$) & 82.2 & 88.6 & 50.6 & 59.7 \\
%         \bottomrule
%         \end{tabular}
%     \caption{$k$-nn accuracies for default and cut-initialized training.}
%     \label{tbl:accuracies}
% \end{table}

\hspace*{-0.7cm}
\begin{minipage}{0.25\textwidth}
    \centering
    \fontsize{7pt}{7pt}\selectfont
    \def\arraystretch{1.165}
    \vspace*{-0.22cm}
    \begin{tabular}{lccc}
        \midrule
         % & & \multicolumn{2}{c}{$k$-nn Accuracy} \\
         & & Top-1 & Top-5 \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{\makecell{\fontsize{5pt}{5pt}\selectfont MoCo\\V2}}} & $c=1$ & 38.7 & 69.7 \\
         & $c=3$ & 43.8 & 71.8 \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{\makecell{\fontsize{5pt}{5pt}\selectfont MoCo\\V3}}} & $c=1$ & 54.8 & 82.7 \\
         & $c=3$ & 58.8 & 86.0 \\
         \midrule
         \multirow{2}{*}{\rotatebox[origin=c]{90}{\makecell{\fontsize{5pt}{5pt}\selectfont DINO}}} & $c=1$ & 43.7 & 76.6 \\
         & $c=3$ & 29.0 & 55.6 \\
         \bottomrule
    \end{tabular}
    \captionof{table}{Imagenet-100 $k$-nn accuracy (epoch 100) for MoCo and Dino.}
    \label{tbl:transformer_accs}
\end{minipage}
\quad
\begin{minipage}{0.42\linewidth}
    \vspace*{-0.04cm}
    \fontsize{8.5pt}{8.5pt}\selectfont
    \centering
    \begin{tabular}{cl cccccc}
    \multicolumn{8}{c}{SimCLR} \\
    \midrule \vspace*{0.1cm}
    & & \multicolumn{6}{c}{Weight Decay} \\
    & & 1e-8 & 1e-7 & \underline{1e-6} & 5e-6 & 1e-5 & 5e-5 \\
    \cmidrule{3-8}
    \multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell{Cut}}} & $c=1$ & 40.8 & 40.4 & 40.5 & 40.9 & 41.5 & 40.4 \\
    & $c=2$ & 42.7 & 42.9 & 42.8 & 42.9 & 42.2 & 40.5 \\
    & $c=4$ & 42.3 & 43.0 & 41.4 & 42.0 & 41.1 & 39.9 \\
    & $c=8$ & 37.1 & 38.8 & 36.8 & 37.9 & 37.3 & 37.3 \\
    \bottomrule
    \end{tabular}
    \captionof{table}{SimCLR $k$-nn accuracy (epoch 100) on Cifar100 for various cut-constants and weight-decays. Default $\lambda$ is underlined.}
    \label{tbl:simclr_wd_cut}
\end{minipage}
\quad
\begin{minipage}{0.3\linewidth}
    \fontsize{8.5pt}{8.5pt}\selectfont
    \vspace*{0.38cm}
    \centering
    \begin{tabular}{cl cccc}
    \multicolumn{6}{c}{SimSiam} \\
    \midrule \vspace*{0.1cm}
    & & \multicolumn{4}{c}{Weight Decay} \\
    & & 5e-5 & 1e-4 & \underline{5e-4} & 1e-3 \\
    \cmidrule{3-6}
    \multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell{Cut}}} & $c=1$ & 36.7 & 38.5 & 40.5 & 44.7 \\
    & $c=2$ & 41.1 & 44.0 & 48.8 & 42.1 \\
    & $c=4$ & 40.2 & 41.2 & 49.8 & 49.1 \\
    & $c=8$ & 44.4 & 46.4 & 50.2 & 53.2 \\
    \bottomrule
    \end{tabular}
    \captionof{table}{SimSiam $k$-nn accuracy (epoch 100) on Imagenet-100 for various values of $c$ and $\lambda$. Default $\lambda$ is underlined.}
    \label{tbl:simsiam_wd_cut}
\end{minipage}

==> Sections/eccv_6_conclusion.tex <==
\section{Conclusion and Open Questions}

In this work, we presented the settings where the cosine similarity loss becomes difficult to optimize. Through theoretical and experimental analysis, we verified that large embedding norms effectively negate a model's ability to learn meaningful self-supervised representations. Thus, we proposed cut-initialization -- a method that, when paired with weight decay, ensures that the embedding-norm effect does not occur.

Nonetheless, there remain unanswered questions. Primarily, it is unclear to us why the attraction-only models benefit so much more from cut-initialization than the contrastive ones. On its surface, the theory should apply to both equally. Furthermore, we have only evaluated the embedding-norm and opposite-halves effects and on image recognition tasks. Although the theory states that the cosine similarity's issues exist regardless of the setting, perhaps some task-specific domains suffer from these issues more than others? We hope we have facilitated further research into the dynamics behind SSL training.

% In this work we identified and analyzed the settings in which the cosine similarity's gradients go to 0 in the context of self-supervised learning. Although we have shown contexts where both the Embedding-Norm and Opposite-Halves effects happen, there remain open questions that were outside the scope of this work. First, is the Opposite-Halves effect more common for datasets with long-tailed, imbalanced class distributions? Preliminary experiments on the Flowers102~\cite{flowers} dataset have implied this to be the case, although it may be that this dataset is susceptible to issues with the choice of augmentations. Second, what are the consequences of using a loss function that has the cosine similarity nested within it (for example, the loss function from~\cite{normface})? By the chain rule, there is an implication that the Embedding-Norm effect must still play a role for the same reasons described in this paper. Expanding on this, there's a natural question of ``how general is the Embedding-Norm effect?'' Are there other loss functions for which it appears? We hope we have opened the door to discussing these questions more thoroughly.


==> Sections/paperflow.tex <==

\textbf{FLOW}
\begin{enumerate}
    \item Abstract: one para

    \item Intro: pure intro, methods, general field stuff: success stories " good models, tasks, and finish it full para of methods that are understanding methods kind of and their issues? or incompleteness. contribution and short easy to understand.

    \item Preliminaries: only talk about models, no in-depth! move 2.2 and 2.3 to "method" - done

    \item Section 3: Method, 3.2 can be L2 norm, 3.1 Gradients - done

    \item Section 4. All experiments in one section: respective heading telling what we are checking? 

    \item Important subsection for above: talking about why we did what we did in experiments, epochs, model choice, parameters, datasets, etc. Justification for choice, through common sense, limited resources, or citing papers that do so. 

    \item Section 5. Discussion section:
    Take away points, what to do to fix things (repeating what we talked about in contributions), and then inconclusive points further where to look at in future papers. 

  

\end{enumerate}
Experiments
\begin{enumerate}
    \item  dino and dinovit on cifar100  -running
    \item mocov2plus, mocov2plus accelerated on cifar100 -running
    \item dino and dinovit on cifar100 with cuts and higher batch-size
    \item mocov2plus, mocov2plus accelerated on cifar100 with cuts and higher batch-size
    \item Above two on imagnet100
   
\end{enumerate}

==> Tables/min_dists_in_batch.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{cccccc}
    \multicolumn{2}{c}{SimCLR} & \multicolumn{2}{c}{SimSiam} & \multicolumn{2}{c}{BYOL} \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
    \makecell{Loss Function} & \makecell{Accuracy} & \makecell{Model Variant} & \makecell{Accuracy} & \makecell{Model Variant} & \makecell{Accuracy} \\
    \midrule
    Only Attractions\, $\left( \mathcal{L}^\mathcal{A} \right)$ & 29\% & \makecell{No Stop Grad.} & 24\% & \makecell{No Predictor} & 23\% \\
    InfoNCE\, $\left( \mathcal{L}^\mathcal{A} + \mathcal{L}^\mathcal{R} \right)$ & 71\% &  \makecell{Default} & 58\% & Default & 56\% \\
    Only Repulsions\, $\left( \mathcal{L}^\mathcal{R} \right)$  & 33\% & \makecell{Default; $\text{WD}=0$} & 34\% & \makecell{Default; $\text{WD}=0$} & 40\% \\
    \end{tabular}
    \caption{Accuracies at epoch 64 of the models trained for Figure~\ref{fig:embed_dists}. Accuracies are obtained by freezing the Resnet-18 backbone (without the projector) and training a single linear layer on its output space.}
    \label{tbl:embed_plot_accuracies}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

